Bilevel parameter learning for higher-order total variation regularisation models

We consider a bilevel optimisation approach for parameter learning in higher-order total variation image reconstruction models. Apart from the least squares cost functional, naturally used in bilevel learning, we propose and analyse an alternative cost, based on a Huber regularised TV-seminorm. Differentiability properties of the solution operator are verified and a first-order optimality system is derived. Based on the adjoint information, a quasi-Newton algorithm is proposed for the numerical solution of the bilevel problems. Numerical experiments are carried out to show the suitability of our approach and the improved performance of the new cost functional. Thanks to the bilevel optimisation framework, also a detailed comparison between TGV$^2$ and ICTV is carried out, showing the advantages and shortcomings of both regularisers, depending on the structure of the processed images and their noise level.

==> highlightname.tex <==
%\addbibresource{\jobname.bib}
\newcommand*{\mknamesignature}[5]{\def#1{#2|#3|#4|#5}}
\mknamesignature{\highlightname}{Valkonen}{Tuomo}{}{}
% mbox needed to not make next character automatically  upper case
\def\shortform{\mbox{\textsl{T.V.}}}
\makeatletter

\DeclareNameFormat{labelname}{%
  \begingroup
  \mknamesignature{\currentsignature}{#1}{#3}{#5}{#7}%
  \ifdefequal{\highlightname}{\currentsignature}%
    {\let\mkbibnamefirst=\@gobble%
     \def\mkbibnamelast{\shortform\@gobble}%
     \let\mkbibnameprefix=\@gobble%
     \let\mkbibnameaffix=\@gobble}%
    {\let\mkbibnamefirst=\@gobble}%
  \ifcase\value{uniquename}%
    \usebibmacro{name:last}{#1}{#3}{#5}{#7}%
  \or
    \ifuseprefix
      {\usebibmacro{name:first-last}{#1}{#4}{#5}{#8}}
      {\usebibmacro{name:first-last}{#1}{#4}{#6}{#8}}%
  \or
    \usebibmacro{name:first-last}{#1}{#3}{#5}{#7}%
  \fi
  \endgroup
  \usebibmacro{name:andothers}%
}

\makeatother


==> img/bsds300/filelist.tex <==
\IM{100075}%
\IM{100080}%
\IM{100098}%
\IM{103041}%
\IM{104022}%
\IM{105019}%
\IM{105053}%
\IM{106020}%
\IM{106025}%
\IM{108041}%
\IM{108073}%
\IM{109034}%
\IM{112082}%
\IM{113009}%
\IM{113016}%
\IM{113044}%
\IM{117054}%
\IM{118020}%
\IM{118035}%
\IM{12003}%
\IM{12074}%
\IM{122048}%
\IM{124084}%
\IM{126039}%
\IM{130034}%
\IM{134008}%
\IM{134052}%
\IM{135037}%
\IM{135069}%
\IM{138032}%
\IM{138078}%
\IM{140055}%
\IM{140075}%
\IM{144067}%
\IM{145014}%
\IM{145053}%
\IM{147021}%
\IM{147062}%
\IM{15004}%
\IM{15088}%
\IM{151087}%
\IM{153077}%
\IM{153093}%
\IM{155060}%
\IM{156079}%
\IM{157036}%
\IM{159029}%
\IM{159045}%
\IM{159091}%
\IM{16052}%
\IM{161062}%
\IM{163014}%
\IM{163062}%
\IM{164074}%
\IM{166081}%
\IM{169012}%
\IM{170054}%
\IM{172032}%
\IM{173036}%
\IM{176019}%
\IM{176035}%
\IM{176039}%
\IM{178054}%
\IM{181018}%
\IM{181079}%
\IM{181091}%
\IM{183055}%
\IM{183087}%
\IM{187003}%
\IM{187029}%
\IM{187039}%
\IM{187071}%
\IM{187083}%
\IM{188005}%
\IM{188063}%
\IM{188091}%
\IM{189003}%
\IM{189011}%
\IM{196015}%
\IM{198004}%
\IM{198023}%
\IM{198054}%
\IM{20008}%
\IM{202012}%
\IM{207056}%
\IM{209070}%
\IM{2092}%
\IM{216041}%
\IM{216053}%
\IM{216066}%
\IM{22013}%
\IM{22090}%
\IM{22093}%
\IM{225017}%
\IM{227040}%
\IM{227046}%
\IM{23025}%
\IM{23080}%
\IM{23084}%
\IM{231015}%
\IM{232038}%
\IM{236017}%
\IM{238011}%
\IM{239007}%
\IM{239096}%
\IM{24004}%
\IM{24063}%
\IM{242078}%
\IM{245051}%
\IM{246016}%
\IM{246053}%
\IM{247085}%
\IM{249061}%
\IM{249087}%
\IM{25098}%
\IM{253036}%
\IM{254033}%
\IM{254054}%
\IM{260081}%
\IM{26031}%
\IM{268002}%
\IM{27059}%
\IM{271008}%
\IM{271031}%
\IM{274007}%
\IM{277095}%
\IM{28075}%
\IM{28096}%
\IM{285036}%
\IM{286092}%
\IM{292066}%
\IM{293029}%
\IM{299091}%
\IM{301007}%
\IM{302003}%
\IM{309004}%
\IM{310007}%
\IM{311068}%
\IM{311081}%
\IM{314016}%
\IM{317080}%
\IM{323016}%
\IM{326038}%
\IM{33066}%
\IM{35008}%
\IM{35010}%
\IM{35058}%
\IM{35070}%
\IM{35091}%
\IM{353013}%
\IM{361084}%
\IM{365025}%
\IM{365073}%
\IM{368016}%
\IM{368078}%
\IM{370036}%
\IM{372047}%
\IM{374020}%
\IM{374067}%
\IM{376001}%
\IM{376020}%
\IM{385028}%
\IM{388016}%
\IM{41004}%
\IM{41025}%
\IM{42044}%
\IM{42078}%
\IM{43070}%
\IM{43083}%
\IM{45077}%
\IM{46076}%
\IM{48055}%
\IM{54005}%
\IM{55067}%
\IM{55075}%
\IM{56028}%
\IM{59078}%
\IM{60079}%
\IM{61060}%
\IM{61086}%
\IM{65010}%
\IM{65019}%
\IM{65074}%
\IM{65132}%
\IM{66039}%
\IM{66075}%
\IM{67079}%
\IM{68077}%
\IM{71046}%
\IM{76002}%
\IM{78019}%
\IM{80099}%
\IM{8049}%
\IM{8143}%
\IM{87065}%
\IM{90076}%
\IM{92059}%
\IM{94079}%
\IM{95006}%
\IM{97017}%


==> resimg/comparison-bsds300-ALL-noise10-huberonly.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{huberonly}-\mathname{tv} & $0.893$ & $0.035$ & $0.897$ & 23 & $31.24$ & $1.87$ & $30.94$ & 23 & $6.7\ee^{4}$ & $2.2\ee^{4}$ & $6.6\ee^{4}$ & 13\\
	\costname{huberonly}-\mathname{ictv} & $0.897$ & $0.034$ & $0.902$ & 142 & $31.36$ & $1.81$ & $31.11$ & 152 & $6.6\ee^{4}$ & $2.2\ee^{4}$ & $6.4\ee^{4}$ & 112\\
	\costname{huberonly}-\mathname{tgv2} & $0.896$ & $0.035$ & $0.901$ & 35 & $31.31$ & $1.88$ & $31.01$ & 25 & $6.6\ee^{4}$ & $2.2\ee^{4}$ & $6.4\ee^{4}$ & 75\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-ALL-noise10-l2.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{l2}-\mathname{tv} & $0.887$ & $0.035$ & $0.889$ & 29 & $31.31$ & $1.50$ & $31.15$ & 25 & $5.72$ & $1.91$ & $5.51$ & 25\\
	\costname{l2}-\mathname{ictv} & $0.889$ & $0.036$ & $0.893$ & 127 & $31.41$ & $1.44$ & $31.28$ & 131 & $5.57$ & $1.83$ & $5.37$ & 131\\
	\costname{l2}-\mathname{tgv2} & $0.888$ & $0.035$ & $0.891$ & 44 & $31.38$ & $1.50$ & $31.20$ & 44 & $5.64$ & $1.90$ & $5.44$ & 44\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-ALL-noise2-huberonly.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{huberonly}-\mathname{tv} & $0.987$ & $0.006$ & $0.988$ & 23 & $42.43$ & $1.07$ & $42.37$ & 23 & $1.7\ee^{4}$ & $3.1\ee^{3}$ & $1.8\ee^{4}$ & 25\\
	\costname{huberonly}-\mathname{ictv} & $0.988$ & $0.006$ & $0.989$ & 135 & $42.56$ & $1.06$ & $42.51$ & 157 & $1.7\ee^{4}$ & $3.3\ee^{3}$ & $1.7\ee^{4}$ & 125\\
	\costname{huberonly}-\mathname{tgv2} & $0.987$ & $0.006$ & $0.989$ & 42 & $42.51$ & $1.09$ & $42.44$ & 20 & $1.7\ee^{4}$ & $3.3\ee^{3}$ & $1.7\ee^{4}$ & 50\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-ALL-noise2-l2.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{l2}-\mathname{tv} & $0.986$ & $0.007$ & $0.987$ & 15 & $42.46$ & $0.95$ & $42.43$ & 24 & $0.42$ & $0.07$ & $0.43$ & 24\\
	\costname{l2}-\mathname{ictv} & $0.987$ & $0.007$ & $0.988$ & 147 & $42.57$ & $0.95$ & $42.56$ & 135 & $0.41$ & $0.07$ & $0.42$ & 135\\
	\costname{l2}-\mathname{tgv2} & $0.987$ & $0.007$ & $0.988$ & 38 & $42.53$ & $0.97$ & $42.51$ & 41 & $0.41$ & $0.07$ & $0.42$ & 41\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-ALL-noise20-huberonly.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{huberonly}-\mathname{tv} & $0.789$ & $0.067$ & $0.798$ & 18 & $27.37$ & $2.13$ & $26.98$ & 24 & $9.4\ee^{4}$ & $3.6\ee^{4}$ & $9.0\ee^{4}$ & 13\\
	\costname{huberonly}-\mathname{ictv} & $0.795$ & $0.065$ & $0.804$ & 143 & $27.46$ & $2.10$ & $27.05$ & 142 & $9.2\ee^{4}$ & $3.6\ee^{4}$ & $8.8\ee^{4}$ & 92\\
	\costname{huberonly}-\mathname{tgv2} & $0.794$ & $0.066$ & $0.804$ & 39 & $27.44$ & $2.12$ & $27.04$ & 34 & $9.2\ee^{4}$ & $3.6\ee^{4}$ & $8.8\ee^{4}$ & 95\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{tgv2} $>$ \mathname{ictv} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{tgv2} $>$ \mathname{ictv} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{tgv2} $>$ \mathname{ictv} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-ALL-noise20-l2.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{l2}-\mathname{tv} & $0.786$ & $0.053$ & $0.790$ & 31 & $27.50$ & $1.71$ & $27.27$ & 33 & $14.11$ & $5.78$ & $13.16$ & 33\\
	\costname{l2}-\mathname{ictv} & $0.790$ & $0.054$ & $0.790$ & 123 & $27.56$ & $1.64$ & $27.37$ & 119 & $13.84$ & $5.54$ & $12.75$ & 119\\
	\costname{l2}-\mathname{tgv2} & $0.789$ & $0.053$ & $0.793$ & 46 & $27.55$ & $1.70$ & $27.33$ & 48 & $13.93$ & $5.73$ & $12.95$ & 48\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-noise10-huberonly.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{huberonly}-\mathname{tv} & $0.898$ & $0.036$ & $0.900$ & 4 & $31.28$ & $1.63$ & $30.97$ & 8 & $7.3\ee^{4}$ & $2.2\ee^{4}$ & $7.3\ee^{4}$ & 1\\
	\costname{huberonly}-\mathname{ictv} & $0.906$ & $0.034$ & $0.909$ & 139 & $31.54$ & $1.68$ & $31.21$ & 142 & $7.1\ee^{4}$ & $2.2\ee^{4}$ & $7.1\ee^{4}$ & 121\\
	\costname{huberonly}-\mathname{tgv2} & $0.905$ & $0.035$ & $0.907$ & 57 & $31.47$ & $1.72$ & $31.10$ & 50 & $7.1\ee^{4}$ & $2.2\ee^{4}$ & $7.1\ee^{4}$ & 78\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-noise10-l2.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{l2}-\mathname{tv} & $0.897$ & $0.033$ & $0.898$ & 9 & $31.54$ & $1.76$ & $31.15$ & 2 & $5.52$ & $1.89$ & $5.51$ & 2\\
	\costname{l2}-\mathname{ictv} & $0.903$ & $0.032$ & $0.903$ & 131 & $31.72$ & $1.76$ & $31.33$ & 148 & $5.30$ & $1.81$ & $5.35$ & 148\\
	\costname{l2}-\mathname{tgv2} & $0.902$ & $0.033$ & $0.903$ & 60 & $31.67$ & $1.80$ & $31.28$ & 50 & $5.38$ & $1.87$ & $5.39$ & 50\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-noise2-huberonly.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	Noisy data & $0.978$ & $0.015$ & $0.981$ & 0 & $41.56$ & $0.86$ & $41.95$ & 0 & $2.1\ee^{4}$ & $2.8\ee^{2}$ & $2.1\ee^{4}$ & 0\\
	\costname{huberonly}-\mathname{tv} & $0.988$ & $0.005$ & $0.989$ & 1 & $42.57$ & $1.10$ & $42.46$ & 5 & $1.7\ee^{4}$ & $3.3\ee^{3}$ & $1.8\ee^{4}$ & 3\\
	\costname{huberonly}-\mathname{ictv} & $0.989$ & $0.005$ & $0.990$ & 141 & $42.74$ & $1.16$ & $42.62$ & 143 & $1.6\ee^{4}$ & $3.5\ee^{3}$ & $1.7\ee^{4}$ & 139\\
	\costname{huberonly}-\mathname{tgv2} & $0.989$ & $0.005$ & $0.989$ & 58 & $42.70$ & $1.17$ & $42.55$ & 52 & $1.6\ee^{4}$ & $3.5\ee^{3}$ & $1.7\ee^{4}$ & 58\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{tgv2} $>$ \mathname{tv} $>$ \mathname{noisy}} & \multicolumn{4}{|c}{\mathname{tgv2} $>$ \mathname{tv} $>$ \mathname{noisy}} & \multicolumn{4}{|c}{\mathname{tgv2} $>$ \mathname{tv} $>$ \mathname{noisy}}\\
\end{tabular}


==> resimg/comparison-bsds300-noise2-l2.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	Noisy data & $0.978$ & $0.015$ & $0.981$ & 0 & $41.56$ & $0.86$ & $41.95$ & 0 & $0.51$ & $0.01$ & $0.51$ & 0\\
	\costname{l2}-\mathname{tv} & $0.988$ & $0.005$ & $0.988$ & 2 & $42.64$ & $1.14$ & $42.50$ & 2 & $0.41$ & $0.08$ & $0.43$ & 2\\
	\costname{l2}-\mathname{ictv} & $0.988$ & $0.005$ & $0.989$ & 142 & $42.79$ & $1.18$ & $42.64$ & 148 & $0.39$ & $0.08$ & $0.41$ & 148\\
	\costname{l2}-\mathname{tgv2} & $0.988$ & $0.005$ & $0.989$ & 56 & $42.76$ & $1.19$ & $42.58$ & 50 & $0.40$ & $0.08$ & $0.42$ & 50\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{tgv2} $>$ \mathname{tv} $>$ \mathname{noisy}} & \multicolumn{4}{|c}{\mathname{tgv2} $>$ \mathname{tv} $>$ \mathname{noisy}} & \multicolumn{4}{|c}{\mathname{tgv2} $>$ \mathname{tv} $>$ \mathname{noisy}}\\
\end{tabular}


==> resimg/comparison-bsds300-noise20-huberonly.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{huberonly}-\mathname{tv} & $0.795$ & $0.063$ & $0.799$ & 7 & $27.27$ & $1.64$ & $27.02$ & 11 & $1.0\ee^{5}$ & $3.5\ee^{4}$ & $9.7\ee^{4}$ & 1\\
	\costname{huberonly}-\mathname{ictv} & $0.810$ & $0.061$ & $0.814$ & 120 & $27.52$ & $1.66$ & $27.24$ & 125 & $9.7\ee^{4}$ & $3.4\ee^{4}$ & $9.6\ee^{4}$ & 79\\
	\costname{huberonly}-\mathname{tgv2} & $0.808$ & $0.062$ & $0.814$ & 73 & $27.50$ & $1.74$ & $27.15$ & 64 & $9.8\ee^{4}$ & $3.5\ee^{4}$ & $9.5\ee^{4}$ & 120\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv}, \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv}, \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv}, \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparison-bsds300-noise20-l2.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
	 & \multicolumn{4}{c}{SSIM} & \multicolumn{4}{|c}{PSNR} & \multicolumn{4}{|c}{value}\\
	\hline
	 & mean & std & med & best & mean & std & med & best & mean & std & med & best\\
	\hline
	\costname{l2}-\mathname{tv} & $0.802$ & $0.056$ & $0.804$ & 8 & $27.70$ & $1.93$ & $27.28$ & 0 & $13.65$ & $5.53$ & $13.14$ & 0\\
	\costname{l2}-\mathname{ictv} & $0.811$ & $0.056$ & $0.816$ & 126 & $27.86$ & $1.91$ & $27.45$ & 138 & $13.14$ & $5.22$ & $12.62$ & 138\\
	\costname{l2}-\mathname{tgv2} & $0.810$ & $0.057$ & $0.814$ & 66 & $27.83$ & $1.94$ & $27.41$ & 62 & $13.28$ & $5.38$ & $12.77$ & 62\\
	\hline
	95\% t-test &\multicolumn{4}{c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}} & \multicolumn{4}{|c}{\mathname{ictv} $>$ \mathname{tgv2} $>$ \mathname{tv}}\\
\end{tabular}


==> resimg/comparisonmatrix-bsds300-ALL-noise10-huberonly.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118035}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{144067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145014}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147021}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147062}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{151087}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{156079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{163014}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{163062}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{20008}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22090}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{22093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{225017}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{227040}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{239007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{242078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{245051}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246016}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254033}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{268002}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{28075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{28096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{285036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{286092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{299091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{310007}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{323016}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{326038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{42044}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{42078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{55067}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{61060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{65074}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{71046}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{8049}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%


==> resimg/comparisonmatrix-bsds300-ALL-noise10-l2.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{118035}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{144067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147021}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{147062}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{151087}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{156079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{163014}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{163062}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{176039}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{183055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198023}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{20008}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22090}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{22093}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{225017}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{227040}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{239007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{24063}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{242078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{245051}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{246016}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{254033}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{268002}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{28075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{28096}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{285036}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{286092}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{299091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{310007}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{323016}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{326038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42044}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{42078}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{55067}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{61060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{65074}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{68077}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{71046}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{76002}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{8049}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%


==> resimg/comparisonmatrix-bsds300-ALL-noise2-huberonly.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{118035}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{144067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145014}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147021}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147062}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{151087}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{156079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{172032}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{176035}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{20008}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22090}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{22093}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{225017}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{227040}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{231015}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{232038}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{239007}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239096}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{245051}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246016}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254033}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{268002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{28075}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{28096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{285036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{299091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{310007}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{323016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{326038}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41025}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{42044}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{42078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{55067}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{60079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{61060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{8049}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{87065}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{90076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%


==> resimg/comparisonmatrix-bsds300-ALL-noise2-l2.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{118035}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{144067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145014}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147021}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147062}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{151087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{156079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{157036}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{176035}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{20008}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22090}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{22093}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{225017}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{227040}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{231015}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{232038}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{239007}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{245051}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254033}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{268002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{277095}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{28075}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{28096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{285036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{299091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{309004}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{310007}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{323016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{326038}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{374020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41025}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{42044}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{42078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{55067}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{61060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{8049}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{8143}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{87065}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{90076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%


==> resimg/comparisonmatrix-bsds300-ALL-noise20-huberonly.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118035}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{144067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145014}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147021}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{147062}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{151087}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{156079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{163062}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{183055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{20008}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22090}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{22093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{225017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227040}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227046}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{239007}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239096}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{245051}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254033}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{268002}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{285036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{299091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{302003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{310007}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{317080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{323016}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{326038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{361084}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42044}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{42078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{55067}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{59078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{60079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{61060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{66075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{67079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{8049}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%


==> resimg/comparisonmatrix-bsds300-ALL-noise20-l2.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{105053}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{118020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{118035}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{144067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145014}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147021}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{147062}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{151087}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{156079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{163014}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{163062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{176039}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{183055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{20008}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22090}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{22093}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{225017}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{227040}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{239007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{24063}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{242078}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{245051}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{246016}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{254033}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{268002}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{277095}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{28096}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{285036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{299091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{310007}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{323016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{326038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35058}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{41025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{42044}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{42078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{46076}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{55067}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{61060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{68077}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{71046}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{76002}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{78019}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{80099}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{8049}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%


==> resimg/comparisonmatrix-bsds300-noise10-huberonly.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{144067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147021}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147062}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{151087}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{156079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{157036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163062}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{20008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22090}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22093}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{225017}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227040}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{245051}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254033}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{268002}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{28075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28096}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{285036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{299091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{310007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{323016}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{326038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{388016}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42044}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{55067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61060}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{8049}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%


==> resimg/comparisonmatrix-bsds300-noise10-l2.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{118035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{144067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147021}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147062}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{151087}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{156079}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{20008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22090}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22093}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{225017}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227040}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{245051}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254033}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{268002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{28075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{285036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{299091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{310007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{323016}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{326038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35010}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{388016}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41025}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{42044}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{42078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{55067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61060}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{67079}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{8049}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%


==> resimg/comparisonmatrix-bsds300-noise2-huberonly.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{118035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{130034}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{144067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145014}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147021}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147062}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{151087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{156079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{20008}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22090}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22093}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{225017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{227040}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239007}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{245051}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254033}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{268002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{28075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28096}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{285036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{286092}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{299091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{310007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311068}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{323016}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{326038}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35010}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42044}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{42078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{55067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61060}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{8049}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%


==> resimg/comparisonmatrix-bsds300-noise2-l2.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{118035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{130034}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{138032}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{144067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145014}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147021}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147062}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{151087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{156079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{157036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{20008}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22090}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22093}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{225017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227040}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239007}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{245051}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254033}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{268002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{28075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28096}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{285036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{299091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{302003}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{310007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311068}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{323016}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{326038}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35010}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{42044}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{55067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61060}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{8049}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{92059}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%


==> resimg/comparisonmatrix-bsds300-noise20-huberonly.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{105053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{122048}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{126039}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{130034}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{135069}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{138032}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{144067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145014}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147021}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147062}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{151087}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{156079}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163062}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tv}{tgv2}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{20008}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22090}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{22093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{225017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227040}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227046}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{245051}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{249087}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254033}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{268002}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{tgv2}{ictv}}}%
\IMX{274007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28096}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{285036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{292066}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{293029}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{299091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{302003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{309004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{310007}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{323016}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{326038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{365025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{374067}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41004}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42044}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{43070}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{46076}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{48055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{54005}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{55067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61060}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{66075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{8049}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{92059}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%


==> resimg/comparisonmatrix-bsds300-noise20-l2.tex <==
\IMX{100075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{100080}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{100098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{103041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{104022}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{105053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{106020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{106025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{108041}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{108073}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{109034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{112082}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{113009}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{113044}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{117054}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{118020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{118035}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{12074}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{122048}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{124084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{126039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{130034}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{134052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135037}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{135069}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{138032}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{138078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{140075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{144067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{145014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{145053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{147021}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{147062}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{15088}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{tv}{ictv}}}%
\IMX{151087}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{153077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{153093}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{155060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{156079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{157036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{159029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159045}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{159091}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{16052}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{161062}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163014}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{163062}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{164074}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{166081}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{169012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{170054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{172032}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{173036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{176035}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{176039}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{178054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181018}{{\IMORDER{ictv}{tv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{181091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{183055}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{183087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187029}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{187071}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{187083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188063}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{188091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{189003}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{189011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{196015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{198023}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{198054}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{20008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{202012}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{207056}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{209070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{2092}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216041}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216053}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{216066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22090}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{22093}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{225017}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227040}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{227046}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{23080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{23084}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{231015}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{232038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{236017}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{238011}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{239096}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{24004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{24063}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{242078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{245051}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{246016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{246053}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{247085}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{249061}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{249087}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{25098}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{253036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254033}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{254054}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{260081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{26031}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{268002}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{27059}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{271031}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{274007}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{277095}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{28075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{28096}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{285036}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{286092}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{292066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{293029}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{299091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{301007}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{302003}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{309004}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{310007}{{\IMORDER{tgv2}{tv}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{311068}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{311081}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{314016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{317080}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{323016}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{326038}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{33066}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35008}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35058}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{35091}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{353013}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{361084}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{365025}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{365073}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{368078}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{370036}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{372047}{{\IMORDER{tv}{ictv}{tgv2}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374020}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{374067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{376001}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{376020}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{385028}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{388016}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{41004}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{41025}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{42044}{{\IMORDER{tv}{tgv2}{ictv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{42078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43070}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{43083}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{45077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{46076}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{48055}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{54005}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{55067}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{55075}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{56028}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{59078}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{60079}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61060}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{61086}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65010}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65019}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{65074}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{65132}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66039}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{66075}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{67079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{68077}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{71046}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{76002}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{78019}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{80099}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{8049}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{8143}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{87065}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{90076}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{92059}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%
\IMX{94079}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{95006}{{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}{\IMORDER{ictv}{tgv2}{tv}}}%
\IMX{97017}{{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}{\IMORDER{tgv2}{ictv}{tv}}}%


==> resimg/ictv-huberonly-bsds300-ALL100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.023}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.017}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{12}%
\gdef\RESdist{3.234}%
\gdef\RESssim{0.844}%
\gdef\RESpsnr{31.388}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-bsds300-ALL100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.001}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{11}%
\gdef\RESdist{0.961}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{41.925}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-bsds300-ALL100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.058}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.064}%
\gdef\RESdist{0.000004}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{11}%
\gdef\RESdist{4.637}%
\gdef\RESssim{0.728}%
\gdef\RESpsnr{28.258}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-bsds300-ALL100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.023}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.017}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{12}%
\gdef\RESdist{1.842}%
\gdef\RESssim{0.877}%
\gdef\RESpsnr{33.283}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-bsds300-ALL100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.001}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{11}%
\gdef\RESdist{0.670}%
\gdef\RESssim{0.973}%
\gdef\RESpsnr{42.067}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-bsds300-ALL100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.058}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.064}%
\gdef\RESdist{0.000004}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{11}%
\gdef\RESdist{2.485}%
\gdef\RESssim{0.859}%
\gdef\RESpsnr{30.682}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-dataset100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.030}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.010}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{17}%
\gdef\RESdist{3.175}%
\gdef\RESssim{0.855}%
\gdef\RESpsnr{31.549}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-dataset100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.003}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.001}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{0.939}%
\gdef\RESssim{0.985}%
\gdef\RESpsnr{42.133}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-dataset100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.056}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.033}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{20}%
\gdef\RESdist{4.591}%
\gdef\RESssim{0.744}%
\gdef\RESpsnr{28.346}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-dataset100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.042}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.064}%
\gdef\RESdist{0.000004}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{9}%
\gdef\RESdist{1.756}%
\gdef\RESssim{0.935}%
\gdef\RESpsnr{33.699}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-dataset100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.005}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.006}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{0.615}%
\gdef\RESssim{0.985}%
\gdef\RESpsnr{42.817}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-dataset100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.094}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.130}%
\gdef\RESdist{0.000008}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{18}%
\gdef\RESdist{2.524}%
\gdef\RESssim{0.902}%
\gdef\RESpsnr{30.548}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-dataset11-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.103}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.505}%
\gdef\RESdist{0.000008}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{23}%
\gdef\RESdist{4.971}%
\gdef\RESssim{0.970}%
\gdef\RESpsnr{34.201}%
\gdef\RESerror{}%


==> resimg/ictv-huberonly-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.051}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.068}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{16}%
\gdef\RESdist{6.656}%
\gdef\RESssim{0.895}%
\gdef\RESpsnr{31.667}%
\gdef\RESerror{}%


==> resimg/ictv-l2-bsds300-ALL100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.018}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.011}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{13}%
\gdef\RESdist{3.198}%
\gdef\RESssim{0.851}%
\gdef\RESpsnr{31.486}%
\gdef\RESerror{}%


==> resimg/ictv-l2-bsds300-ALL100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.001}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{0.944}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{42.080}%
\gdef\RESerror{}%


==> resimg/ictv-l2-bsds300-ALL100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.045}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.032}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{4.632}%
\gdef\RESssim{0.738}%
\gdef\RESpsnr{28.268}%
\gdef\RESerror{}%


==> resimg/ictv-l2-bsds300-ALL100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.018}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.011}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{13}%
\gdef\RESdist{2.180}%
\gdef\RESssim{0.804}%
\gdef\RESpsnr{31.818}%
\gdef\RESerror{}%


==> resimg/ictv-l2-bsds300-ALL100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.001}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{0.715}%
\gdef\RESssim{0.967}%
\gdef\RESpsnr{41.503}%
\gdef\RESerror{}%


==> resimg/ictv-l2-bsds300-ALL100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.045}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.032}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{3.102}%
\gdef\RESssim{0.728}%
\gdef\RESpsnr{28.756}%
\gdef\RESerror{}%


==> resimg/ictv-l2-dataset100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.026}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.010}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{14}%
\gdef\RESdist{3.172}%
\gdef\RESssim{0.856}%
\gdef\RESpsnr{31.558}%
\gdef\RESerror{}%


==> resimg/ictv-l2-dataset100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.001}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{16}%
\gdef\RESdist{0.939}%
\gdef\RESssim{0.985}%
\gdef\RESpsnr{42.135}%
\gdef\RESerror{}%


==> resimg/ictv-l2-dataset100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.051}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.034}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{9}%
\gdef\RESdist{4.570}%
\gdef\RESssim{0.743}%
\gdef\RESpsnr{28.384}%
\gdef\RESerror{}%


==> resimg/ictv-l2-dataset100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.031}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.038}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{1.662}%
\gdef\RESssim{0.931}%
\gdef\RESpsnr{34.175}%
\gdef\RESerror{}%


==> resimg/ictv-l2-dataset100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.004}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.005}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{15}%
\gdef\RESdist{0.602}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{43.000}%
\gdef\RESerror{}%


==> resimg/ictv-l2-dataset100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.070}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.094}%
\gdef\RESdist{0.000006}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{2.379}%
\gdef\RESssim{0.896}%
\gdef\RESpsnr{31.060}%
\gdef\RESerror{}%


==> resimg/ictv-l2-dataset11-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.049}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.056}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{3.947}%
\gdef\RESssim{0.965}%
\gdef\RESpsnr{36.206}%
\gdef\RESerror{}%


==> resimg/ictv-l2-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.041}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.051}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{6.439}%
\gdef\RESssim{0.887}%
\gdef\RESpsnr{31.954}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-bsds300-ALL100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.024}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.027}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{3.266}%
\gdef\RESssim{0.840}%
\gdef\RESpsnr{31.303}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-bsds300-ALL100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.002}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{12}%
\gdef\RESdist{0.973}%
\gdef\RESssim{0.983}%
\gdef\RESpsnr{41.822}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-bsds300-ALL100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.059}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.080}%
\gdef\RESdist{0.000005}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{11}%
\gdef\RESdist{4.642}%
\gdef\RESssim{0.727}%
\gdef\RESpsnr{28.249}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-bsds300-ALL100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.024}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.027}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{1.774}%
\gdef\RESssim{0.891}%
\gdef\RESpsnr{33.610}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-bsds300-ALL100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.002}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{12}%
\gdef\RESdist{0.659}%
\gdef\RESssim{0.974}%
\gdef\RESpsnr{42.204}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-bsds300-ALL100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.059}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.080}%
\gdef\RESdist{0.000005}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{11}%
\gdef\RESdist{2.459}%
\gdef\RESssim{0.866}%
\gdef\RESpsnr{30.775}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-dataset100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.024}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.025}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{22}%
\gdef\RESdist{3.261}%
\gdef\RESssim{0.841}%
\gdef\RESpsnr{31.316}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-dataset100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.000}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{17}%
\gdef\RESdist{0.947}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{42.056}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-dataset100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.060}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.043}%
\gdef\RESdist{0.000003}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{16}%
\gdef\RESdist{4.625}%
\gdef\RESssim{0.736}%
\gdef\RESpsnr{28.281}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-dataset100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.041}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.056}%
\gdef\RESdist{0.000003}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{15}%
\gdef\RESdist{1.699}%
\gdef\RESssim{0.940}%
\gdef\RESpsnr{33.984}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-dataset100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.005}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.006}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{0.595}%
\gdef\RESssim{0.987}%
\gdef\RESpsnr{43.098}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-dataset100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.093}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.139}%
\gdef\RESdist{0.000008}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{14}%
\gdef\RESdist{2.458}%
\gdef\RESssim{0.907}%
\gdef\RESpsnr{30.775}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-dataset11-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.071}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.453}%
\gdef\RESdist{0.000007}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{17}%
\gdef\RESdist{3.769}%
\gdef\RESssim{0.989}%
\gdef\RESpsnr{36.606}%
\gdef\RESerror{}%


==> resimg/tgv2-huberonly-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.051}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.069}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{12}%
\gdef\RESdist{6.615}%
\gdef\RESssim{0.897}%
\gdef\RESpsnr{31.720}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-bsds300-ALL100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.019}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.019}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{6}%
\gdef\RESdist{3.237}%
\gdef\RESssim{0.846}%
\gdef\RESpsnr{31.381}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-bsds300-ALL100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.001}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{13}%
\gdef\RESdist{0.956}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{41.975}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-bsds300-ALL100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.046}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.056}%
\gdef\RESdist{0.000003}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{4.659}%
\gdef\RESssim{0.732}%
\gdef\RESpsnr{28.217}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-bsds300-ALL100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.019}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.019}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{6}%
\gdef\RESdist{2.105}%
\gdef\RESssim{0.816}%
\gdef\RESpsnr{32.122}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-bsds300-ALL100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.001}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{13}%
\gdef\RESdist{0.705}%
\gdef\RESssim{0.968}%
\gdef\RESpsnr{41.629}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-bsds300-ALL100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.046}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.056}%
\gdef\RESdist{0.000003}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{2.990}%
\gdef\RESssim{0.743}%
\gdef\RESpsnr{29.074}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-dataset100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.021}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.010}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{13}%
\gdef\RESdist{3.202}%
\gdef\RESssim{0.852}%
\gdef\RESpsnr{31.475}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-dataset100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.000}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{17}%
\gdef\RESdist{0.947}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{42.061}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-dataset100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.054}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.038}%
\gdef\RESdist{0.000002}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{13}%
\gdef\RESdist{4.591}%
\gdef\RESssim{0.742}%
\gdef\RESpsnr{28.345}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-dataset100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.032}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.041}%
\gdef\RESdist{0.000003}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{12}%
\gdef\RESdist{1.623}%
\gdef\RESssim{0.937}%
\gdef\RESpsnr{34.380}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-dataset100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.004}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.005}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{7}%
\gdef\RESdist{0.583}%
\gdef\RESssim{0.986}%
\gdef\RESpsnr{43.269}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-dataset100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.072}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.093}%
\gdef\RESdist{0.000006}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{9}%
\gdef\RESdist{2.338}%
\gdef\RESssim{0.906}%
\gdef\RESpsnr{31.211}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-dataset11-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.055}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.307}%
\gdef\RESdist{0.000005}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{19}%
\gdef\RESdist{3.603}%
\gdef\RESssim{0.986}%
\gdef\RESpsnr{36.997}%
\gdef\RESerror{}%


==> resimg/tgv2-l2-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.041}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.058}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{11}%
\gdef\RESdist{6.412}%
\gdef\RESssim{0.890}%
\gdef\RESpsnr{31.992}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-bsds300-ALL100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.025}%
\gdef\RESdist{0.000192}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{3.262}%
\gdef\RESssim{0.839}%
\gdef\RESpsnr{31.313}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-bsds300-ALL100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.003}%
\gdef\RESdist{0.000020}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{0.975}%
\gdef\RESssim{0.983}%
\gdef\RESpsnr{41.807}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-bsds300-ALL100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.061}%
\gdef\RESdist{0.000478}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{4.643}%
\gdef\RESssim{0.726}%
\gdef\RESpsnr{28.248}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-bsds300-ALL100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.025}%
\gdef\RESdist{0.000192}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{1.919}%
\gdef\RESssim{0.873}%
\gdef\RESpsnr{32.926}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-bsds300-ALL100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.003}%
\gdef\RESdist{0.000020}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{0.715}%
\gdef\RESssim{0.970}%
\gdef\RESpsnr{41.507}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-bsds300-ALL100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.061}%
\gdef\RESdist{0.000478}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{2.664}%
\gdef\RESssim{0.836}%
\gdef\RESpsnr{30.077}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-dataset100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.025}%
\gdef\RESdist{0.000197}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{13}%
\gdef\RESdist{3.274}%
\gdef\RESssim{0.838}%
\gdef\RESpsnr{31.283}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-dataset100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESdist{0.000014}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{11}%
\gdef\RESdist{0.954}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{41.995}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-dataset100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.070}%
\gdef\RESdist{0.000545}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{4.739}%
\gdef\RESssim{0.713}%
\gdef\RESpsnr{28.070}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-dataset100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.074}%
\gdef\RESdist{0.000576}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{6}%
\gdef\RESdist{2.306}%
\gdef\RESssim{0.895}%
\gdef\RESpsnr{31.331}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-dataset100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.007}%
\gdef\RESdist{0.000051}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{9}%
\gdef\RESdist{0.690}%
\gdef\RESssim{0.981}%
\gdef\RESpsnr{41.805}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-dataset100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.180}%
\gdef\RESdist{0.001408}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{3.633}%
\gdef\RESssim{0.817}%
\gdef\RESpsnr{27.383}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-dataset11-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.136}%
\gdef\RESdist{0.000532}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{6}%
\gdef\RESdist{5.521}%
\gdef\RESssim{0.966}%
\gdef\RESpsnr{33.291}%
\gdef\RESerror{}%


==> resimg/tv-huberonly-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.057}%
\gdef\RESdist{0.000221}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{10}%
\gdef\RESdist{6.944}%
\gdef\RESssim{0.887}%
\gdef\RESpsnr{31.298}%
\gdef\RESerror{}%


==> resimg/tv-l2-bsds300-ALL100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.019}%
\gdef\RESdist{0.000149}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{3.245}%
\gdef\RESssim{0.845}%
\gdef\RESpsnr{31.360}%
\gdef\RESerror{}%


==> resimg/tv-l2-bsds300-ALL100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESdist{0.000016}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{0.958}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{41.961}%
\gdef\RESerror{}%


==> resimg/tv-l2-bsds300-ALL100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.047}%
\gdef\RESdist{0.000367}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{4.679}%
\gdef\RESssim{0.730}%
\gdef\RESpsnr{28.180}%
\gdef\RESerror{}%


==> resimg/tv-l2-bsds300-ALL100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.019}%
\gdef\RESdist{0.000149}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{2.205}%
\gdef\RESssim{0.804}%
\gdef\RESpsnr{31.720}%
\gdef\RESerror{}%


==> resimg/tv-l2-bsds300-ALL100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESdist{0.000016}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{0.754}%
\gdef\RESssim{0.964}%
\gdef\RESpsnr{41.046}%
\gdef\RESerror{}%


==> resimg/tv-l2-bsds300-ALL100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.047}%
\gdef\RESdist{0.000367}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{8}%
\gdef\RESdist{3.127}%
\gdef\RESssim{0.723}%
\gdef\RESpsnr{28.687}%
\gdef\RESerror{}%


==> resimg/tv-l2-dataset100075noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.021}%
\gdef\RESdist{0.000164}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{3.233}%
\gdef\RESssim{0.845}%
\gdef\RESpsnr{31.391}%
\gdef\RESerror{}%


==> resimg/tv-l2-dataset100075noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.002}%
\gdef\RESdist{0.000012}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{10}%
\gdef\RESdist{0.952}%
\gdef\RESssim{0.984}%
\gdef\RESpsnr{42.008}%
\gdef\RESerror{}%


==> resimg/tv-l2-dataset100075noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.055}%
\gdef\RESdist{0.000430}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{13}%
\gdef\RESdist{4.615}%
\gdef\RESssim{0.732}%
\gdef\RESpsnr{28.300}%
\gdef\RESerror{}%


==> resimg/tv-l2-dataset100080noise10-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.033}%
\gdef\RESdist{0.000256}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{9}%
\gdef\RESdist{1.808}%
\gdef\RESssim{0.911}%
\gdef\RESpsnr{33.446}%
\gdef\RESerror{}%


==> resimg/tv-l2-dataset100080noise2-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.005}%
\gdef\RESdist{0.000036}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{23}%
\gdef\RESdist{0.663}%
\gdef\RESssim{0.980}%
\gdef\RESpsnr{42.161}%
\gdef\RESerror{}%


==> resimg/tv-l2-dataset100080noise20-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.072}%
\gdef\RESdist{0.000561}%
\gdef\RESdimX{128}%
\gdef\RESdimY{128}%
\gdef\RESiters{5}%
\gdef\RESdist{2.599}%
\gdef\RESssim{0.861}%
\gdef\RESpsnr{30.294}%
\gdef\RESerror{}%


==> resimg/tv-l2-dataset11-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.052}%
\gdef\RESdist{0.000202}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{4.157}%
\gdef\RESssim{0.948}%
\gdef\RESpsnr{35.756}%
\gdef\RESerror{}%


==> resimg/tv-l2-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.042}%
\gdef\RESdist{0.000163}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{12}%
\gdef\RESdist{6.623}%
\gdef\RESssim{0.879}%
\gdef\RESpsnr{31.710}%
\gdef\RESerror{}%


==> resumesubequations.tex <==

\usepackage{etoolbox}

\makeatletter
\newcounter{qrr@oldeq}
\newcounter{qrr@oldsubeq}
\newcounter{qrr@realeq}
\renewenvironment{subequations}{%
  \refstepcounter{equation}%
  \protected@edef\theparentequation{\theequation}%
  \setcounter{parentequation}{\value{equation}}%
  \setcounter{equation}{0}%
  \def\theequation{\theparentequation\alph{equation}}%
  \ignorespaces
}{%
  \setcounter{qrr@oldeq}{\value{parentequation}}%
  \setcounter{qrr@oldsubeq}{\value{equation}}%
  \setcounter{equation}{\value{parentequation}}%
  \ignorespacesafterend
}
\newenvironment{resumesubequations}{%
  \setcounter{qrr@realeq}{\value{equation}}%
  \let\theparentequation\theequation%
  \patchcmd{\theparentequation}{equation}{parentequation}{}{}%
  \setcounter{parentequation}{\numexpr\value{qrr@oldeq}-1}%
  \setcounter{equation}{\value{qrr@oldsubeq}}%
  \def\theequation{\theparentequation\alph{equation}}%
  \refstepcounter{parentequation}%
  \ignorespaces
}{%
  \setcounter{qrr@oldeq}{\value{parentequation}}%
  \setcounter{qrr@oldsubeq}{\value{equation}}%
  \setcounter{equation}{\value{qrr@realeq}}%
  \ignorespacesafterend
}
\makeatother


==> symbols-ip.tex <==

\usepackage{undertilde}

\newcommand{\jprod}{\circ}
\newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\iK}{\interior \K}
\newcommand{\E}{\mathcal{E}}
\newcommand{\Neigh}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\nullspace}[1]{\mathcal{N}(#1)}
\newcommand{\iprod}[2]{\langle #1,#2\rangle}
\newcommand{\Pep}{P_e^\perp}
\newcommand{\DC}{\mathrm{DC}}
\newcommand{\extsubdiff}{\widehat \subdiff}
\newcommand{\subdiffDC}{\subdiff^\DC}
\newcommand{\extsubdiffDC}{\extsubdiff^\DC}
\newcommand{\polar}[1]{{#1}^\circ}
\newcommand{\bipolar}[1]{{#1}^{\circ\circ}}
\newcommand{\regnormal}{\widehat N}
\newcommand{\regtangent}{\widehat T}
\newcommand{\HG}{{\widehat G}}
\newcommand{\HU}{{\widehat U}}
\newcommand{\IG}{\inv G}
\newcommand{\IHG}{\inv \HG}
\newcommand{\varsym}{\bullet}
\newcommand{\wtilde}{\widetilde}
\newcommand{\setto}{\rightrightarrows}

\renewcommand{\norm}[1]{\|#1\|}
\newcommand{\adjnorm}[1]{\left\|#1\right\|}

\newcommand{\eigval}{\zeta}
\newcommand{\eigvaltwo}{\sigma}

\newcommand{\Arw}{\mathrm{Arw}}


==> symbols-mna.tex <==

\newcommand{\mna}{\phi}
\newcommand{\plusmna}{\oplus}
\newcommand{\minusmna}{\ominus}
\newcommand{\iprodmna}{\odot}
%\DeclareMathOperator{\plusmna}{\hat +}
%\DeclareMathOperator{\minusmna}{\hat{--}}
%\DeclareMathOperator{\iprodmna}{\hat \times}
\newcommand{\Rmna}{\R_\mna}
\newcommand{\maybeeq}{\stackrel{?}{=}}
\newcommand\rhodom\sqsubset
\newcommand\rhodominv\sqsupset
\newcommand\rhodomneq{\sqsubset_{!}}
\newcommand\rholub\sqcup
\newcommand\rhoglb\sqcap
\newcommand{\sumop}{\biguplus}
\newcommand{\sumz}{\biguplus}
\newcommand{\plusz}{\uplus}
\newcommand{\minusz}{\uminus}
\newcommand{\pz}{\zeta}

